Bipartite Graphs as Models of Complex Networks

It appeared recently that the classical random graph model used to represent real-world complex networks does not capture their main properties. Since then, various attempts have been made to provide accurate models. We study here a model which achieves the following challenges: it produces graphs which have the three main wanted properties (clustering, degree distribution, average distance), it is based on some real-world observations, and it is sufficiently simple to make it possible to prove its main properties. This model consists in sampling a random bipartite graph with prescribed degree distribution. Indeed, we show that any complex network may be viewed as a bipartite graph with some specific characteristics, and that its main properties may be viewed as consequences of this underlying structure. We also propose a growing model based on this observation.

==> network.tex <==
\newcommand{\CNS}
{Complex Networks}

\newcommand{\cns}
{complex networks}

\newcommand{\cn}
{complex network}

\newcommand{\network}
{network}

\newcommand{\networks}
{networks}

\newcommand{\link}
{link}

\newcommand{\links}
{links}

\newcommand{\nodes}
{nodes}

\newcommand{\node}
{node}

\newcommand{\cc}
{clustering coefficient}


